Schema-Free Dependency Parsing via Sequence Generation

Dependency parsing aims to extract syntactic dependency structure or semantic dependency structure for sentences. Existing methods suffer the drawbacks of lacking universality or highly relying on the auxiliary decoder. To remedy these drawbacks, we propose to achieve universal and schema-free Dependency Parsing (DP) via Sequence Generation (SG) DPSG by utilizing only the pre-trained language model (PLM) without any auxiliary structures or parsing algorithms. We first explore different serialization designing strategies for converting parsing structures into sequences. Then we design dependency units and concatenate these units into the sequence for DPSG. Thanks to the high flexibility of the sequence generation, our DPSG can achieve both syntactic DP and semantic DP using a single model. By concatenating the prefix to indicate the specific schema with the sequence, our DPSG can even accomplish multi-schemata parsing. The effectiveness of our DPSG is demonstrated by the experiments on widely used DP benchmarks, i.e., PTB, CODT, SDP15, and SemEval16. DPSG achieves comparable results with the first-tier methods on all the benchmarks and even the state-of-the-art (SOTA) performance in CODT and SemEval16. This paper demonstrates our DPSG has the potential to be a new parsing paradigm. We will release our codes upon acceptance.

==> section/0.abstract-Luo.tex <==
\begin{abstract}
% There are two mainstream methods for dependency parsing and semantic dependency parsing: transition-based method and graph-based method. Most research of these two methods achieve the outstanding performance. However, the performance of these two methods in in-domain parsing is limited by the ability of model structure. Some research investigate the parser combing the pre-trained language model such as BERT, but the pre-trained model used by transition-based method or graph-based method. In this paper, we propose an generated-based method for dependency parsing by pre-trained language model.
Dependency parsing is to extract syntactic dependency structure or semantic dependency structure for sentence.
Existing methods suffer the drawbacks of lacking universality or highly relying on auxiliary decoder.
%Existing methods face the challenges of universality lacking and auxiliary decoder.
To remedy these drawbacks, we propose to achieve universal and schema-free dependency parsing (DP) via sequence generation (SG) \model~by utilizing only the pre-trained language model~(PLM) but not any auxiliary structure or parsing algorithms.
We explore different serialization designing strategies for converting parsing structures into sequences. Then we design \textit{dependency pair} and concatenate these pairs with the sequence for DPSG.
Thanks to the high flexibility of the generated sequence, our DPSG can achieve both syntactic DP and semantic DP using a single model.
By concatenating the prefix indicating specific schema with the sequence, our DPSG can even accomplish the multi-schema parsing.
The effectiveness of our DPSG are demonstrated by the experiments on widely used DP benchmarks, i.e. PTB, CODT, SDP15 and SemEval16.
Our DPSG achieve comparable results with the first tier methods on all the benchmarks, and even the state-of-the-art (SOTA) performance in CODT and SemEval16.
% Previous seq2seq dependency parsing methods treat parsing as sequence labeling. 
% In this paper, we propose achieve schema- dependency parsing as sequence generation by pre-trained language model without any additional structure.
% Our DPSG can accomplish syntactic dependency parsing and semantic dependency parsing in different schema such as in-domain parsing and cross-domain parsing.
% Our DPSG even can achieve cross-schema training and multi-schema training by one set of parameters.

% We validate the effectiveness of our method by conducting experiments on PTB, CODT, SDP15 and, SDP15 and SemEval16. The results demonstrate our method significantly outperform previous seq2seq parsing methods and achieve SOTA or comparable performance to SOTA on these datasets.
\end{abstract}



==> section/1.introduction-Luo.tex <==
\section{Introduction}

% \emph{syntactic} or \emph{semantic}
Dependency Parsing (DP), which aims to extract the structural information beneath sentences, is fundamental in understanding natural languages.
It benefits a wide range of natural language processing (NLP) applications, such as information extraction~\cite{attardi2014ie}, machine translation~\cite{bugliarello2020mt}, question answering~\cite{teney2017qa}, and information retrieval~\cite{chandurkar2017ir}.
As illustrated in Figure~\ref{fig:parsingtree}, dependency parsing predicts for each word the existence and dependency relation with all the other words according to a pre-defined schema.
Such dependency structure is represented in tree or directed acyclic graph, which can be converted into flattened sequence, as presented in this paper.

% 应该再增加一句，与图片对应，说明如图所示，我们可以直观地看到，这两类结构是可以被序列化的，这样在开头就点出了工作的重点

% Recently, there are two main threads in DP studies.
% One thread further subdivides DP into more specific tasks or optimizes DP in various data-scarce situation. 
% \citet{someone} start to consider semantic dependency relation beyond the syntactic dependency relation.
% \citet{someone} highlight the importance of language-specific features.
% % and introduce cross-lingual DP task.
% \citet{someone} argue that dependency relation should be domain-invariant and propose cross-domain DP task.
% The other thread engineers more sophisticated parsing modules. 
% With the promising external knowledge encoded by Pre-trained Language Models (PLM), a large amount of studies~\cite{something} successfully verifies the effectiveness of incorporating contextual embeddings~\cite{bert, roberta}.
% There are also efforts to leverage cross-domain (-lingual) dependency knowledge with transfer learning techniques.
% These two threads are inter-winded and motivate the development of each other, 

\begin{figure}[t]
\centering
    \includegraphics[width=1.0\linewidth]{figures/fig1-demo-v2.pdf}
\caption{
% This sentence "Ms. Haag plays Elianti ." is from Penn Treebank3. StanFord means the syntactic parsing tree convert from StanfordNLP. DM, PAS and PSD are three different schema of semantic dependency graph.
% Two different dependency structures of the same sentence ``\textit{Ms. Haag plays Elianti .}''.
% The presented syntactic dependency structure adopts the Stanford schema~\cite{manning2014stanford} and the semantic dependency structure follows the PSD schema~\cite{stephan2015sdp15}.
Parsing ``\textit{Ms. Haag plays Elianti .}'' according to the Stanford syntactic dependency structure~\cite{manning2014stanford} and the PSD semantic dependency structure~\cite{stephan2015sdp15}.
They are further converted into the unified serialized representations using our method.
}
\label{fig:parsingtree}
\end{figure}

% % lin
% However, most previous research for DP focus on transition-based methods and graph-based methods.
% Altougth outstanding performance, these methods also need the auxiliary traditional parsing algorithms, which make the parsing process cubersome.
% %% 变得越来越繁琐
% On the other hand, the usage of PLM is narrowd in replacing the original embedding layer to get a better word representation.

% In this paper, we propose treat dependency parsing as sequence generation.
% By Serializing parsing structure, the workflow of DP change into a seq-2-seq paradigm.
% The input of our method is the original sequence, and the output is the serialization of the parsing structure.
% To get the high-quality serialization sequence and fully utilize the potential of PLM, we use T5 and mT5 as the backbone to generate the parsing sequence.


Dependency parsing prospers with many subdivided tasks to better serve downstream applications.
% On one hand, new schemata are proposed for syntactic and semantic dependency parsing~\cite{li2003sdp,stephan2015sdp15,che2016semeval}.
For example, recent works extend dependency parsing from syntactic relations to semantic relations with many new schemata~\cite{li2003sdp,stephan2015sdp15,che2016semeval,zhang2019broad,fernandez2020transition}.
Besides, corpora from different domains facilitate the research on cross-domain dependency parsing~\cite{li2019codt,li2019bert}.
More recently, with the development of pre-trained language models (PLMs), researchers manage to enable PLMs on dependency task, and successfully achieve the new state-of-the-art results~\cite{mahovy2017neural,ma2018stackptr,zhang2019broad,gan21mrc}.
% with sophisticated parser, such as neural maximum spanning tree~\cite{mahovy2017neural}, pointer network~\cite{ma2018stackptr}, and biaffine network~\cite{gan21mrc}.
%这里的描述和后面decoder有些重复了，能否删去，直接总说PLM的应用给parsing带来了提升，具体的parser留到decoder那一段
% These methods achieve the new state-of-the-art results.
However, there are still two main issues.

% In recent years, studies in dependency parsing prosper with many subdivided tasks to better serve down stream applications.
% \citet{li2003sdp,stephan2015sdp15,che2016semeval} introduce the semantic dependency parsing task which move from the analysis of syntactic structure to sentence semantics.
% There are also efforts to overcome the data-scarcity problem via cross-domain training and transfer learning~\cite{li2019codt}.
% More recently, after the birth of pre-trained langauge models (PLMs), 
% % the birth of pre-trained language models (PLM) sheds lights on dependency parsing.
% it has been shown effective to use the pre-trained contextualized representations with an elaborated parser, such as bi-affine decoder~\cite{gan21mrc}, pointer network~\cite{ma2018stackptr}, neural MST~\cite{mahovy2017neural}, and achieves the new state-of-the-art results on dependency parsing.
% However, there still remains two challenges.


\textbf{Relying on Extra Decoder.}
Previous parsers usually produce the parsing results by employing an extra decoding module, such as biaffine network for score calculation~\cite{gan21mrc} and neural transducer for decision making~\cite{zhang2019broad}.
These modules cannot be pre-trained and learn the dependency knowledge merely from the training corpora. This prevents them from generalizing to sentences of either different domains or different schemata.
% learn the dependency knowledge that could bias towards the training corpus.
% Thus, they are less transferable to directly parse sentences from a different domain.
%\boda{and also leads to the lacking of universality}

\textbf{Lack of Universality.}
Although there are many successful parsers, most of them are schema-specific.
For example, machine reading comprehension based parsers~\cite{gan21mrc} are only suitable for syntactic dependency parsing.
Besides, they require re-training before being adapted to another schema, which is extremely costly for the PLM based parsers.
% Both parsers with PLMs and without PLMs can achieve outstanding performances on parsing task.
% But most of them are schema-speific models.
\boda{Need more details, such as parameters}.
In addition, most existing parsers require auxiliary pseudo-labeling processes or domain adaptation modules when applied to unsupervised cross-domain parsing tasks.
\boda{I will add citations later}

% \textbf{Lack of Universality.} There are lots of data schemata in DP, but it is difficult to parsing them using one model.
% There are mainly three types of methods towards dependency parsing: 
% Graph-based dependency parsers calculate the dependency score for each pair of words in the sentence~\cite{kiperwasser2016bilstm,dozat2017biaffine}.
% % However, it requires to search for a heuristic threshold when the number of head words is non-determinant, which is not accurate.
% They search a non-accurate threshold when there are multiple head words.
% Sequence labelling based methods tag the head word for each word in the sentence~\cite{strzyz2019viable,vacareanu2020pat}.
% These two methods are not designed for non-determinant number of head words.
% Transition-based models~\cite{zhang2019broad,fernandez2020transition} read sentence word by word and make decisions at the current word.
% Although they give accurate decisions when there are multiple head words, they are limited as they use localized information.



% \textbf{Lack of Generality.}
% % It is difficult to design a single model that performs generally well on all the subdivided dependency tasks.
% % There are mainly two gaps.
% There are mainly two gaps that preserves a single parser from performing generally well on all the subdivided tasks.
% % First, different dependency schema can allow for either exactly one head word (in syntactic dependency parsing) or multiple head words (in semantic dependency parsing) for each dependent word.
% First, different dependency schema may have different constraint for the number of head words. 
% Syntactic dependency relation usually requires each word has exactly one head word, while semantic dependency parsing usually allows for an indeterminate number of head words.
% Current attempts for the multiple head words schema usually search for a heuristic threshold to determine for each word whether it is a head word.
% Secondly, an extra domain adaptation procedure is usually required for parsing data from different domains.
% Some recent researches suggest that PLMs may have the born-in cross-domain capability~\cite{peng2019nlpcc}. 





% % \textbf{Architecture Engineering.}
% \textbf{Relying on Extra Decoder.}
% The PLMs based parsers usually leverage an extra decoder to undertake the responsibility for the dependency knowledge and use PLMs as the input embeddings. 
% These modules further complicate the model and make the fine-tuning objective inconsistent with the pre-training objective.
% % introduce a gap between the fine-tuning stage and the pre-training stage.
% Besides, as a series of probing works suggest that PLMs themselves capture certain structural knowledge, we hypothesis that such extra decoder may not be necessary~\cite{clark2019bert,hewitt2019probe}. (can cause human bias)

% 核心贡献是 
% 1. 用 Seq2Seq 解决 DP, 通过任务的重新定义解决了这些问题（重点在 idea 和思路，为什么可以解决以前的问题）
% 2. 另起一段说我们的核心方法，输入的 prompt，单纯的文本输入缺乏输入位置信息，而这种位置信息是非常重要的，单纯用 Seq2Seq 的方法不好学，注重 motivation。Parsing 的结果是个树的结构，无法直接用在 Seq2Seq 的模型上。和输出的 serialization

To address these issues, 
we propose schema-free \textbf{D}ependency \textbf{P}arsing via \textbf{S}equence \textbf{G}eneration (\model).
% and use a single encoder-decoder pre-trained language model to directly generate the dependency structure as a sequence.
The core idea is to find a unified unambiguous serialized representation for both syntactic and semantic dependency structures.
Then an encoder-decoder PLM is learned to generate the parsing results using the serialized representation, without the need for additional decoder.
That is, our parser can achieve its function using an original PLM (without any modification), and thus is completely pre-trained.
% Furthermore, the unified representation provides a principled way to pack different schemata into a single model.
Furthermore, by adding a prefix to the serialized representation, \model~provides a principled way to pack different schemata into a single model.
% The PLM takes on the role of dependency parser, and are completely pre-trained.
% The serialized representation directly encodes how many head words there are for each dependent word, rather than using a heuristic threshold to decide for each word whether it is a head word.
% In this way, a single encoder-decoder pre-trained language model can generate the parsing results in sequences alone, without the need for additional decoders.
% This prones potential bias towards the dependency knowledge in the training dataset domain.
% and could be less biased towards the dependency knowledge in the training dataset domain.

In particular, \model~consists of three key components.
The \textit{Serializer} is responsible for converting the dependency structure to serialized representation.
The \textit{Positional Prompt} scheme provides supplementary position information in the input sentence to facilitate the sequence generation process.
The \textit{encoder-decoder PLM} together with added special tokens performs the parsing task by simply extracting the results from the generated sequence.
% Special tokens are added to the vocabulary of an encoder-decoder PLM, and the PLM undertakes the parsing task via sequence generation.
% A encoder-decoder PLM with additional special tokens to generate the results.



% To address the two challenges, we propose to cast \textbf{D}ependency \textbf{P}arsing as \textbf{S}equence \textbf{G}eneration (\model) and use a single encoder-decoder pre-trained language model to directly generate the dependency structure as a sequence.
% We first design a one-to-one mapping between the dependency structure and a novel serialized representation, where we append to each word the position of its head word and their dependency relation.
% % Words are repeated if they have multiple head words in semantic dependency parsing.
% For semantic dependency parsing, we repeat words that have multiple head words.
% Then we design a prompt for the input sentence, which supplies the positional information for each word.
% Finally, an encoder-decoder PLM is fine-tuned to take the prompted sentences as input and generate the serialized sequence as output.
% The serialization provides an accurate portrayal for multiple head words, \model~bridges the gap between different dependency schema.
% As the sequence generation is undertaken by the PLM's decoder, \model~is able to use a fully pre-trained model, and could be less biased towards the dependency knowledge in the training dataset domain.

% There are many benefits to adopt \model.
% \model~directly determines the number of head words for each word as it generates the results.
% It also requires no extra decoding module.
% Two rules, word to dependency information, dependency information to words.


We conduct experiments on four popular DP benchmarks: PTB~\cite{??}, CODTB~\cite{??}, SDP15B~\cite{??} and SemEval16B~\cite{??}. The results show that our~\model~performs generally well on both syntactic and semantic dependency parsing tasks.
The performance of \model~significantly outperforms the baselines on Chinese cross-domain syntactic (CODT) and Chinese semantic dependency parsing (SemEval16) corpora, and achieves comparable results on the other two benchmarks.
Our method can even be trained to parse multiple different schemata using only one set of parameters.
A series of exploratory experiments suggest that \model~is also optimal for engineering practice.
% to provide the optimal engineering practice.

% To address the two challenges, we propose to cast \textbf{D}ependency \textbf{P}arsing as \textbf{S}equence \textbf{G}eneration (DPSG) and use a single sequence-to-sequence (Seq2Seq) pre-trained language model to directly generate the results.
% In particular, we design a serialized representation for the dependency structure, where each word is followed by the position of and the relation with its head word.
% % If a dependent word has multiple head word, it is repeated multiple times, each with a different head word position.
% Dependent word having multiple head words is repeated multiple times in the serialized representation, each corresponding to a different head word position.
% We inject positional prompt to the input sentence, and use the serialized representation as the target to fine-tune the pre-trained Seq2Seq language model.
% The final dependency structure can be easily recovered with the positional and the relational information in the output sequence.
% A series of analysis experiments are conducted to verify the optimal engineering 
% that our provided serialization scheme is optimal among several possible choices.

% experimental results.
% We also conducted a series of analysis experiments to verify the optimal engineering solution.

% We conduct experiments on 4 sets of datasets to examine the performance of DPSG under different subdivided parsing tasks.
% DPSG significantly outperforms previous methods on Chinese cross-domain syntactic dependency parsing (CODT1) and semantic dependency parsing (SemEval16).
% It also achieves comparable performance with other PLM based method on the rest datasets without introducing specialized neural module or training procedure.

% Our results suggest that 


% These experimental results suggest that


% Provide two insights.
% 1. sequence generation is more general and is suitable for both.
% 2. PLM is a parser, no extra module is needed.



% \vpara{Key Points}

% 1. First Generated-base

% 2. (First) Universal Parsing Work (almost directly in all settings without any code changes, the only thing need to do is preprocess original data format to serialization format)

% 3. SOTA

% 4. T5 without auxiliry structure (also drop the auliliry parsing algorithm such MST in graph-based method)

% 5. The adventage of T5-generate:
% 	a. for SeDP, the graph decoding problem
% 	b. (TODO:) for Chinese DP, the parsing from raw text (real end2end, seq2seq)

% \vpara{Key Points Extention:}

% 1. Our method is the first generate-based method for Dependency Parsing. Alough still following the idea of seq2seq, our method directly generate the words and its parsing labeling which is different from previous seq2seq methods belong into sequenece labeling.

% 2. Our method accomplish the universal dependency parsing in in-domain, cross-domain and multi-lingual setting for SyDP and SeDP. Our work is also the first work try to unify these sub-tasks of DP by one method.

% 3. Our method achieve the SOTA performance in many settings of DP.

% 4. Our method use T5 and mT5 without any auxiliary structure and traditional parsing algorithms used in transition-based methods and graph-based methods, whcih simplified the work flow of DP. The pre-label of pos tagging is also dropped. The results also demonstrate that the PLM without auxiliary structure is a parser itself. This observation also provide another way of using PLM in dependency parsing.

% 5. By using genreation-based method, the decoding problem in SeDP is disappeared. Our method is also very suitable for the DP for raw text of Chinese. Comparing with the previous joint model for this scenario, our method do not need making adapt to character-level arc, using generation PLM in this scenario is concise and effective.





% Syntactic Dependency Parsing (\sydp) focuses on extracting the grammar functional relation between words and Semantic Dependency Parsing (\sedp) extracts the semantic relation. Another difference between \sydp and \sedp is the loop restriction, which means one word has one in-arc in \sydp except root word does not have the in-arc. In \sedp, each word may have multiple in-arc or do not located in semantic dependency graph.
% % It serves as one of the fundamental tasks to understand natural languages, and has shown great importance to many NLP tasks, such as xxxx.

% Recent years have witnessed the great success of deep learning, especially pre-trained language models.


% % Dependency parsing is one of the most important task in Natural Language Processing (NLP). There are two types of dependency parsing: Syntactic Dependency Parsing (DP) which focus on extracting the grammar functional relation between words and Semantic Dependency Parsing (SDP) which focus on extracting semantic relation between words. The result of DP and SDP is called "syntactic dependency tree" and "semantic dependency graph", which are shown like Fig \ref{fig:parsingtree}. 

% In addition the to the different relations, the biggest difference in the formation of DP and SDP is that DP generate a tree and SDP generate a graph. In SDP, some words such as comma may have no head word and other words such as noun may have multiple head words. This phenomenon also induce difficulty for methods used in DP.
% % 还应该补充DP和SDP的具体区别，DP只允许树，而SDP允许图的存在


% The mainstream methods for dependency parsing are transition-based method and graph-based method. These methods need post-processing algorithm to get the final parsing result. Comparing with transition-based methods and graph-based methods, seq2seq methods \cite{li2018seq2seq, strzyz2019viable} do not need traditional parsing algorithms or auxiliary structures. But previous seq2seq methods also meet two problems: 1) the low performance of previous seq2seq methods make this technique is impractical. 2) the previous seq2seq methods are type of sequence labeling, the model predict the head tagging and relation tagging. The stable formation involving difficult when the word do not have head word or have multiple head word, which is usual in SDP.


% % Compared with transition-based methods and graph-based methods, seq2seq methods attract less attention.
% % \citet{li2018seq2seq} proposed using seq2seq model to predicate the parsing tagging sequence. \citet{strzyz2019viable} explore more encodings to represent dependency parsing tree and achieve better performance. Their methods are both the sequence labeling type. It is difficult for labeling method to predict the non-label or multi-label when applied in SDP.

% In this paper, we follow the idea of seq2seq parsing and further propose treat dependency parsing as sequence generation. By generation process, our method can easily treat the non-head or multiple-head problem in SDP. We propose use pre-trained language model T5 and mT5 to generate parsing sequence directly.
% Our model can directly used in DP and SDP with in-domain setting and cross-domain setting, which is the universal dependency parsing.




% Our main contributions of this paper are summarized as follows:

% 1) To the best of our knowledge, this is first work treat dependency parsing as sequence generation. We also explore the influence of different 

% 2) Compare with the transition-based method and graph-based method, our method do not meet the decoding problem in SDP, which can be directly used in SDP.

% 3) Our model using the Pre-trained Language Model itself to generate parsing sequence without any parser structure such as Biaffine \cite{dozat2017biaffine} or StackPTR. The result demonstrate the PTM itself is a parser.

% \clearpage



==> section/discussion.tex <==
learning view:
我们的全新范式不仅仅在于标注式与生成式的区别，更在于，直接略去了传统的data->parser->learning中的parser
人工设计的parser结构是没有必要的

语法的形式化表述


实质上和幼儿的模仿习得语言过程有相似之处，父母并不会直接告诉孩子具体的句法规则，而是由孩童在大量的模仿过程中自发习得的，换句话说，在教师特意讲授语法规则前，儿童完全能说出流畅、合乎语法规则的句子，但是他并不能明确地指出具体的句法规则，他说话的能力完全来自模仿
而我们要做的就是让模型这个“儿童”通过模仿生成的句子，能通过简单的规则就直接解析出句法

我们将句法结构重新表征为序列（句子），生成式模型的target就是样句，input是原句，模型并不是在显示地习得parsing structure或者parsing knowledge，而是通过模仿的方式（由生成式语言模型的loss约束），直接学习我们希望他所输出的句子形态，而这种形态下的句子（从定义好的parsing structure转化而来）天然地蕴藏有句法信息

既往的method：

original sentence -> model -> 句法结构

现在的method：

sentence -> model -> sentence (蕴含句法)

通用性即来源于此，因为句法是人类对语言现象的归纳总结，来自于语言，因此通过适当的序列化手段，我们总可以让句法以范式的形式直接被句子表征出来，而利用seq2seq的模型是可以不变的，我们只需要提供不同的句子让模型模仿习得即可，无需再针对特定的句法设计特定的范式


IFT 之前的方法fine-tune时还是无法利用target domain训练后面的decoder


用扩写的方式表达文法
用重写的方式表达文法

==> tables/exp.result.bracket.tex <==
\begin{table}[t]
\centering
\scalebox{0.98}{
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{lccc}
    \toprule
    Metric & \model & Prufer & Bracket\\
    \midrule
    UAS & $96.48$ & $-$ & $-$ \\
    LAS & $95.04$ & $84.92$ & $92.71$ \\
    \bottomrule
    \end{tabular}
}
\caption{Results on PTB for Serializer Designing}
\label{tab:exp:bracket:result}
\end{table}


==> tables/exp.result.schema.tex <==
% the results are not the final results
\begin{table}[t]
    \centering
    \scalebox{1.}{
        \begin{tabular}{cccccccccccccc}
        \toprule
        Dataset & Metric & Alone & Multi-Schema \\
        \midrule
        \multirow{2}{*}{PTB3} 
        & UAS & $96.48$ & $96.30$ \\
        & LAS & $95.04$ & $94.85$\\
        \midrule
        \multirow{2}{*}{DM} 
        & IID & $93.96$ & $94.35$\\
        & OOD & $90.47$ & $90.60$\\
        \midrule
        \multirow{2}{*}{PAS} 
        & IID & $94.26$ & $96.22$\\
        & OOD & $92.38$ & $92.20$\\
        \midrule
        \multirow{2}{*}{PSD} 
        & IID & $81.98$ & $82.25$\\
        & OOD & $80.04$ & $79.65$\\
        \bottomrule
        \end{tabular}
    }
    \caption{Results on Multi-Schema}
    \label{tab:exp:multi-schema}
\end{table}


==> tables/exp.result.sdp15.id.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|r|r|r|r}
    \toprule
     & DM & PAS & PSD & AVG \\
    \midrule
    % Du et al. & 89.1 & 91.3 & 75.7 & 85.3 \\
    % Alme & 89.4 & 91.7 & 77.6 & 86.2 \\
    Wang & 90.3 & 91.7 & 78.6 & 86.9 \\
    % Peng & 90.4 & 92.7 & 78.5 & 87.2 \\
    Dozat & 93.7 & 93.9 & 81.0 & 89.5 \\
    Che & 92.9{\color{white}0} & 94.4{\color{white}0} & 81.6{\color{white}0} & 89.6{\color{white}0} \\
    BERT & 94.57 & 96.13 & 86.80 & 92.50 \\
    % XLNET & 94.2 & 94.8 & 82.7 & 90.57 \\
    % ACE & 95.6 & 95.8 & 83.8 & 91.73 \\
    Ours & 93.96 & 94.26 & 81.98 & 89.99 \\
    \bottomrule
    \end{tabular}
    \caption{Results on SDP15}
    \label{tab:exp:sdp15:result:id}
\end{table}

==> tables/exp.result.sdp15.ood.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c|c|c}
    \toprule
     & DM & PAS & PSD & AVG \\
    \midrule
    % Du et al. & 81.8 & 87.2 & 73.3 & 80.8 \\
    % Alme & 83.8 & 87.6 & 76.2 & 82.5 \\
    Wang & 84.9 & 87.6 & 75.9 & 82.8 \\
    % Peng & 85.3 & 89.0 & 76.4 & 83.6 \\
    Dozat & 88.9 & 90.6 & 79.4 & 86.3 \\
    Che & 89.2 & 92.4 & 81.0 & 87.5 \\
    BERT & 90.86 & 94.38 & 79.48 & 88.21 \\
    % XLNET & 94.2 & 94.8 & 82.7 & 88.6 \\
    % ACE & 92.6 & 94.6 & 83.4 & 90.2 \\
    Ours & 90.47 & 92.38 & 80.04 & 87.63 \\
    \bottomrule
    \end{tabular}
    \caption{Results on SDP15}
    \label{tab:exp:sdp15:result:ood}
\end{table}

==> tables/exp.result.ud.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    \multirow{2}{*}{ }& \multicolumn{2}{l}{\makecell[c]{NEWS}}
     & \multicolumn{2}{l}{\makecell[c]{TEXT}} \\
     & UF & LF & UF & LF\\    
    Dounar & 77.64 & 59.06 & 82.41 & 68.59 \\
    Wang & 81.14 & 63.30 & 85.71 & 72.92 \\
    BERT & 82.92 & 67.27 & 91.10 & 80.41 \\
    Ours & 84.31 & 70.82 & 90.97 & 82.36 \\
    \bottomrule
    \end{tabular}
    \caption{Result on SemEval16}
    \label{tab:sem16:result}
\end{table}
